Thermovoltaic Effects of van der Waals Heterojunctions based on Inert Conductor/Solution Interfaces

It is found that if the inert conductor P has a larger electron work function $\phi$ and surface state function G than the inert conductor N, the inert conductor P and the inert conductor N are isolated by a separator and then immersed in the solution S (abbreviation: inert conductorP$\mid$solutionS$\mid$inert conductorN, or as P$\mid$S$\mid$N). Excluding the electrochemical reaction and thermoelectric effect of P$\mid$S$\mid$N, etc., it is measured that the voltage between the two conductors after the open circuit continues to increase to a certain stable maximum value. Then, the current after the closed-circuit continues to decrease to a certain stable minimum value. Analysis of the structure and properties of P$\mid$S$\mid$N shows that the inert conductor/solution interface relies on physical adsorption to construct van der Waals heterojunctions and that two van der Waals heterojunctions of different potentials form a P-N junction for P$\mid$S$\mid$N. The inert conductors P and N have different potentials. This electric field energy is expressed in the outer circuit when the circuit is open, due to the joint action of the electron work function $\phi$ and the surface state function G, P$\mid$S$\mid$N generates a larger built-in electric field and obtains a larger voltage. When the circuit is closed, P$\mid$S$\mid$N only has the effect of the surface state function G, which produces a smaller built-in electric field, results in a smaller voltage and current. This Thermoelectric conversion phenomenon is called the thermovoltaic effect.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


